Automatic Mixed-Precision Quantization Search of BERT

Pre-trained language models such as BERT have shown remarkable effectiveness in various natural language processing tasks. However, these models usually contain millions of parameters, which prevents them from practical deployment on resource-constrained devices. Knowledge distillation, Weight pruning, and Quantization are known to be the main directions in model compression. However, compact models obtained through knowledge distillation may suffer from significant accuracy drop even for a relatively small compression ratio. On the other hand, there are only a few quantization attempts that are specifically designed for natural language processing tasks. They suffer from a small compression ratio or a large error rate since manual setting on hyper-parameters is required and fine-grained subgroup-wise quantization is not supported. In this paper, we proposed an automatic mixed-precision quantization framework designed for BERT that can simultaneously conduct quantization and pruning in a subgroup-wise level. Specifically, our proposed method leverages Differentiable Neural Architecture Search to assign scale and precision for parameters in each sub-group automatically, and at the same time pruning out redundant groups of parameters. Extensive evaluations on BERT downstream tasks reveal that our proposed method outperforms baselines by providing the same performance with much smaller model size. We also show the feasibility of obtaining the extremely light-weight model by combining our solution with orthogonal methods such as DistilBERT.

==> body/abstract.tex <==
\begin{abstract}

Configurable model size is crucial to the deployment of heavy BERT based models in practice.
Recent techniques on BERT model compression is designed for extreme compacted BERT models, yet these approaches suffer from significant accuracy drop. Quantization is a model-agnostic approach that is able to reduce memory usage and improve inference speed. However, existing approaches cannot automatically optimize the accuracy based on given model size constraint during deployment. In this paper, we tackle the problem to maximize the BERT based model accuracy for a given model size using mixed-precision quantization.
We propose an Differential Neural Architecture Search based method NAS-BERT to search the optimal precision and weights for each parameter in BERT based models, which enables quantization and pruning at the same time in an end-to-end manner. In particular, we use group-wise quantization scheme to allow each tensor to have different scales and precision for each sub group. Moreover, by enabling a search space of 0 bit quantization, we enable the network to automatically pruning out redundant groups of parameters.
We extensively test our proposed NAS-BERT method using different BERT backbone networks on downstream tasks of GLUE tasks and SQuAD and find it outperform existing methods.
%\cz{[confirm if this is correct] Even worse, these approaches cannot automatically optimize the accuracy even when the model size requirement is relaxed.} In this paper, we tackle the problem to maximize the BERT based model accuracy for a given model size. 
% Unlike existing approaches, \kmethod does not need hand-craft adjustments for different model size requirements.
% With the recent introduction of Transformer models, the compression of heavy BERT based models has attracted more and more research attentions.
% Network quantization, as one of the most hardware friendly techniques on low-power mobile devices, has not been widely studied.
% The most relevant work \cite{shen2019q} quantize BERT models using second order Hessian information to determine the precision of each parameter.

\end{abstract}

==> body/backup_introduction.tex <==
\section{Introduction}
Although pre-trained Transformer based language models, such as BERT, have significantly improved the performance in many Natural Language Processing (NLP) tasks, it is challenging to deploy BERT to resource-constrained devices having tight power budgets, due to Transformers' huge essential computing and memory overhead, e.g., an inference of BERT-Base~\cite{lan2019albert} involves $110M$ weights and $29G$ floating point operations.
    
Several approaches such as pruning~\cite{gordon2020compressing,kovaleva2019revealing,michel2019sixteen,voita2019analyzing}, distillation~\cite{sanh2019distilbert,sun2019patient,sunmobilebert,jiao2019tinybert} and optimized architecture compression~\cite{lan2019albert,zhao2019extreme,chen2020adabert} are proposed to reduce the computing and memory overhead of BERT. Transformer and network quantization~\cite{hubara2017quantized,shen2019q,zafrir2019q8bert,banner2019post,chen2019metaquant,stock2019and,fan2020training,lou2019autoq} becomes one of the most hardware friendly BERT acceleration techniques by approximating real-valued weights and activations to fixed-point representations, and performing inferences using cheaper fixed-point multiple-accumulation (MAC) operations. 


Traditional quantization methods use the same bits for the whole BERT-based model~\cite{zafrir2019q8bert}, but different layers have different parameters redundancy and requires different hardware memory capacity, it is necessary to adapt \textit{mixed-precision} quantization for different layers. How to decide a quantization bit for each layer is the most important task of the \textit{mixed-precision} network quantization, since the quantization bit has a large impact on the inference accuracy, latency and hardware overhead. Determining a quantization bit for each layer by hand-crafted heuristics is so sophisticated that even machine learning experts can obtain only sub-optimal results. Instead of using one quantization bit for the whole BERT model, the state-of-the-art \textit{mixed-precision} network quantization Q-BERT~\cite{shen2019q} assigns more quantization bits for layers with larger-eigenvalue parameters. However, since the layers in BERT are not independent and parameters eigenvalues are of high variance with respect to different dataset inputs and models, Q-BERT suffers from significant accuracy loss (2.3\% accuracy degradation) via this hand-crafted \textit{mixed-precision} quantization policies when a small targeted model is needed. As BERT-based models architecture become deeper and more complex, the design space for \textit{mixed-precision} quantization increases exponentially, which is hard to be solved by heuristic, hand-crafted methods. We need a automatic, fast and accurate \textit{mixed-precision} quantization to compress BERT.  


We propose an NAS based method \kmethod that enables differentiable mechanism to search the optimal precision and weights for each parameter in BERT based models. \ys {\kmethod advantages. Unlike existing approaches, \kmethod does not need hand-craft adjustments for different model size requirements.}

\ys {\kmethod technique summary. Unlike existing approaches, \kmethod does not need hand-craft adjustments for different model size requirements.}


\ys {\kmethod technique contributions and results. Unlike existing approaches, \kmethod does not need hand-craft adjustments for different model size requirements. We extensively test our...}




==> rebuttal.tex <==
\section{Rebuttal}

==> title.tex <==
\title{Configurable Memory Size BERT Models via \\ Mixed Precision Quantization Search}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\author{%
  David S.~Hippocampus\thanks{Use footnote for providing further information
    about author (webpage, alternative address)---\emph{not} for acknowledging
    funding agencies.} \\
  Department of Computer Science\\
  Cranberry-Lemon University\\
  Pittsburgh, PA 15213 \\
  \texttt{hippo@cs.cranberry-lemon.edu} \\
  % examples of more authors
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \AND
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
}
